Volumetric 3D Point Cloud Attribute Compression: Learned polynomial bilateral filter for prediction

We extend a previous study on 3D point cloud attribute compression scheme that uses a volumetric approach: given a target volumetric attribute function $f : \mathbb{R}^3 \mapsto \mathbb{R}$, we quantize and encode parameters $\theta$ that characterize $f$ at the encoder, for reconstruction $f_{\hat{\theta}}(\mathbf(x))$ at known 3D points $\mathbf(x)$ at the decoder. Specifically, parameters $\theta$ are quantized coefficients of B-spline basis vectors $\mathbf{\Phi}_l$ (for order $p \geq 2$) that span the function space $\mathcal{F}_l^{(p)}$ at a particular resolution $l$, which are coded from coarse to fine resolutions for scalability. In this work, we focus on the prediction of finer-grained coefficients given coarser-grained ones by learning parameters of a polynomial bilateral filter (PBF) from data. PBF is a pseudo-linear filter that is signal-dependent with a graph spectral interpretation common in the graph signal processing (GSP) field. We demonstrate PBF's predictive performance over a linear predictor inspired by MPEG standardization over a wide range of point cloud datasets.

==> 1-framework.tex <==

We denote $f:\mathbb{R}^3\rightarrow\mathbb{R}$ as a volumetric function defining an attribute field over $\mathbb{R}^3$, the extension to vector attributes is straightforward.
Then, a point cloud can be seen as samples of $f$, with attributes $y_i=f(\mathbf{x}_i)$, where $\x_i \in \mathbb{R}^3$ is sample $i$'s 3D position. To code the attributes given the positions, RAHT($p$) projects $f$ onto a nested sequence of function spaces $\mathcal{F}_0^{(p)}\subseteq\cdots\subseteq\mathcal{F}_L^{(p)}$. 
Each function space $\mathcal{F}_l^{(p)}$ is a parametric family of functions spanned by a set of basis functions $\{\phi_{l,\mathbf{n}}^{(p)}:\mathbf{n}\in\mathcal{N}_l\}$, namely the volumetric B-spline basis functions $\phi_{l,\mathbf{n}}^{(p)}(\mathbf{x})=\phi_{0,\mathbf{0}}^{(p)}(2^l\mathbf{x}-\mathbf{n})$ of order $p$ and scale $l$ for offsets $\mathbf{n}\in\mathcal{N}_l\subset\mathbb{Z}^3$.  
Specifically, for $p=1$, $\phi_{0,\mathbf{0}}^{(p)}(\mathbf{x})$ is the product of ``box'' functions $1_{[0,1]}(x)$ over components $x$ of $\mathbf{x}$, while for $p=2$, it is the product of ``hat'' functions $1_{[-1,1]}(x)(1-|x|)$ over components $x$ of $\mathbf{x}$.

Thus, RAHT(1) projects $f$ onto the space $\mathcal{F}_l^{(1)}$ of functions that are \textit{piecewise constant} over blocks of width $2^{-l}$, while RAHT(2) projects $f$ onto the space $\mathcal{F}_l^{(2)}$ of continuous functions that are \textit{piecewise trilinear} over blocks of width $2^{-l}$. 
In any case, it is clear that $f_l\in\cF_{l}$ implies $f_l\in\cF_{l+1}$ so that the spaces are nested.  
In this paper, we will sometimes omit the order $(p)$ for ease of notation. We define $\bPhi_l=[\phi_{l,\mathbf{n}}]$ as the row-vector of basis functions $\phi_{l,\mathbf{n}}$. Then any $f_l \in \mathcal{F}_l$  can be expressed as a linear combination of basis functions $\phi_{l,\mathbf{n}}$:
% \vspace{-2ex}
\begin{equation} 
f_l(\mathbf{x}) = \sum_{\mathbf{n}\in\mathcal{N}_l} F_{l, \mathbf{n}} \phi_{l, \mathbf{n}}(\mathbf{x}) ,
% \vspace{-0.75ex}
\end{equation}
which may also be written as $f_l=\bPhi_l F_l$

Followed from previous works \cite{do2023volumetric}, we project $f$ on $\mathcal{F}_l$ in the Hilbert space of (equivalence classes of) functions with inner product $\langle f,g\rangle=\sum_if(\mathbf{x}_i)g(\mathbf{x}_i)$. 
Thus, the projection $f_l^*$ of $f$ on $\mathcal{F}_l$ minimizes the squared error $||f-f_l||^2=\langle f-f_l,f-f_l\rangle=\sum_i(y_i-f_l(\mathbf{x}_i))^2$.
Further, the coefficients $F_{l}^*$ that represent the function $f_l^* = f\circ\mathcal{F}_l$ in the basis $\bPhi_l$ can be calculated via the \textit{normal} equation:
% \vspace{-1ex}
\begin{equation} \label{eq:normal_equation_F}
F_{l}^* = (\bPhi_{l}^{\top} \bPhi_{l})^{-1} \bPhi_{l}^{\top} f .
% \vspace{-1ex}
\end{equation}
Here, $\bPhi^\top_{l} f$ denotes the length-$N_l$ vector of inner products $[\langle\phi_{l,\mathbf{n}},f\rangle]$, and $\bPhi_{l}^{\top} \bPhi_{l}$ denotes the $N_l\times N_l$ \textit{Gram matrix} of inner products. According to Pythagorean Theorem \cite[Sec.~3.3]{Luenberger:69}, all the {\em residual} functions
% \vspace{-1ex}
\begin{equation}
    g_l^* = f_{l+1}^* - f_l^*
    % \vspace{-1ex}
\end{equation}
belong to the subspace $\mathcal{G}_l$ which is the orthogonal complement subspace to $\mathcal{F}_l$ in $\mathcal{F}_{l+1}$. Then we have,
% \vspace{-1ex}
\begin{eqnarray}
\cF_L & = &\cF_0 \oplus \cG_0 \oplus \cdots \oplus \cG_l \oplus \cdots \cG_{L-1}   \;\;\; \mbox{and}
\label{eq:sum_of_subspaces} \\
% \end{equation}
% \begin{equation}
f_L^* & = & f_0^* + g_0^* + \cdots + g_l^* + \cdots + g_{L-1}^* .
% \vspace{-2ex}
\label{eqn:fg0_gL}
\end{eqnarray}
We consider the resolution $L$ is high enough such that we take $f_L^*(\mathbf{x}_i)=f(\mathbf{x}_i)$, we then code $f$ by coding $f_0^*$, $g_0^*,\ldots,g_{L-1}^*$.  
To code these functions, we represent them as coefficients in a basis, which are quantized and entropy coded.  Next we show how to compute these coefficients efficiently.


\subsection{Low-pass coefficients}
\label{sec:low_pass_coefs}
Assume that there is a sufficiently fine resolution $L$ such that the $i$th basis function $\phi_{L,\mathbf{n}_i}$ is 1 on $\mathbf{x}_i$ and 0 on $\mathbf{x}_j$ for $j\neq i$, namely $\phi_{L,\mathbf{n}_i}(\mathbf{x}_j)=\delta_{ij}$.  
Then, we have $\bPhi_L^\top \bPhi_L = \I$.
Next, denote by $\A_{l}=[a_{ij}^l]$ a $N_{l} \times N_{l + 1}$ matrix whose $i$th row expresses the $i$th basis function $\phi_{l,\mathbf{n}_i}$ of $\mathcal{F}_l$ in terms of the basis functions $\phi_{l+1,\mathbf{m}_j}$ of $\mathcal{F}_{l+1}$, namely
% \vspace{-1ex}
\begin{equation}
\phi_{l,\mathbf{n}_i} = \sum_j a_{ij}^l \phi_{l+1,\mathbf{m}_j}.
\label{eq:two_scale_eq}
% \vspace{-1ex}
\end{equation}
Note that for $\mathbf{d}_{ij}=\mathbf{m}_j-2\mathbf{n}_i$, we parameterize $\A_{l}$ by a vector of size $3\times 3 \times 3 = 27$ as follow, 
% \vspace{-1ex}
\begin{equation}
a_{ij}^l = \left\{\begin{array}{ll}
w_{\mathbf{d}_{ij}} & \mbox{if}~~ \mathbf{d}_{ij} \in \{-1, 0, 1\}^3 \\ 
0 & \mbox{otherwise}
\end{array}\right.
\label{eq:RAHTp}
% \vspace*{-2ex}
\end{equation}
In \cite{do2023volumetric}, we thoroughly explored two special cases of matrix $\A_{l}$, where $p=1$ and $p=2$.
In vector form, equation \eqref{eq:two_scale_eq} can be re-written as
% \vspace*{-1ex}
\begin{equation}
\bPhi_l = \bPhi_{l+1} \A_l^\top ,
\label{eqn:Phi_ell_in_terms_of_Phi_ell1}
% \vspace*{-1ex}
\end{equation}
where $\mathbf{A}_l$ is an space-invariant but {\em sparse} convolutional matrix with $2\times$ spatial downsampling, and $\mathbf{A}_l^\top$ is the corresponding transpose convolutional matrix with $2\times$ upsampling.  Using these, we can compute matrices of inner products of basis functions from level $l+1$ to level $l$: 
\begin{eqnarray}
\bPhi_l^\top \bPhi_l & = & \A_l\bPhi_{l+1}^\top \bPhi_{l+1} \A_l^\top 
\label{eqn:PhiTPhi}
\end{eqnarray}
Here, the matrix $\bPhi_l^\top \bPhi_l $ is also a sparse convolutional matrix, though space-varying, corresponding to the edge weights of a graph with 27-neighbor connectivity (including self-loops). 

We implement the operation $\bPhi_l^\top \bPhi_l$ by creating a graph of $N_{l}$ nodes, edge weights between node $i$ and node $j$ are calculated using equation \eqref{eqn:PhiTPhi}. So, applying the operation to any length-$N_{l}$ vector would involve only broadcasting the input to the edges $ij$ and aggregation summation at node $i$. Similarly, operation $\A_{l}$ are also implemented as a graph connecting from $N_{l}$ nodes to $N_{l + 1}$ nodes.
In addition, given $\A_{l}$ and $\A_{l}^\top$ are defined as above and $\bPhi_{l+1}^\top \bPhi_{l+1}$ can be represented in $N_{l+1} \times 27$ tensor form, we define \textit{geometric attention} operation $\mathbf{\Gamma}_l$ applying on $\bPhi_{l+1}^\top \bPhi_{l+1}$ as follow,
\begin{eqnarray}
\mathbf{\Gamma}_l(\bPhi_{l+1}^\top \bPhi_{l+1}) & = & \A_l\bPhi_{l+1}^\top \bPhi_{l+1} \A_l^\top 
\label{eqn:GeoAttPhiTPhi}
\end{eqnarray}
Then, it is possible to see that $\mathbf{\Gamma}_l$ a sparse convolution with a space-invariant $3^3 27^2$ kernel directly derived from the $3\times 3 \times 3$ kernel of $\A_{l}$.

Thus, beginning at the highest level of detail $L$, where $\phi_{L,\mathbf{n}_i}(\mathbf{x}_j)=\delta_{ij}$ and $\bPhi_L^\top\bPhi_L=\I$, we have $\bPhi_L^\top f=[y_i]$ and hence (from \eqref{eq:normal_equation_F}) $F_L^*=(\bPhi_L^\top\bPhi_L)^{-1}\bPhi_L^\top f=[y_i]$.  
Moving to $l<L$, we have
\begin{align}
F_l^* & = (\bPhi_l^\top \bPhi_l)^{-1} \bPhi_l^\top f_{l+1}^* \\
& = (\bPhi_l^\top \bPhi_l)^{-1} \bPhi_l^\top \bPhi_{l+1} F_{l+1}^* 
\label{eqn:Fl} \\
& = (\bPhi_l^\top \bPhi_l)^{-1} \A_l(\bPhi_{l+1}^\top \bPhi_{l+1}) F_{l+1}^*.
\label{eqn:F_ell_star_from_F_ell1_star}
\end{align}
Letting $\tilde{F}_l^* = (\bPhi_{l}^\top \bPhi_{l}) F_{l}^*$, which we call un-normalized low-pass coefficients,
we can easily calculate $\tilde{F}_l^*$ for all levels $l$ as
\vspace{-1ex}
\begin{equation}
\tilde{F}_l^* = \A_l \tilde{F}_{l+1}^* .
\label{eqn:analysis_lowpass}
\vspace{-1ex}
\end{equation}
This is an ordinary sparse convolution.
Finally, $F_l^*$ can be computed:
% \vspace{-1ex}
\begin{equation}
    F_l^* = (\bPhi_{l}^\top \bPhi_{l})^{-1} \tilde{F}_l^*.
    \label{eqn:normalization}
% \vspace{-1ex}
\end{equation}
As done in \cite{do2023volumetric}, we will use Pth order Taylor expansion of $x^{-1}$ to compute this as a sub feed-forward network. Later on, these Taylor coefficient will be further optimized in a training process introduced in sec.(\ref{sec:results}).

